Pixel-Wise Prediction based Visual Odometry via Uncertainty Estimation

This paper introduces pixel-wise prediction based visual odometry (PWVO), which is a dense prediction task that evaluates the values of translation and rotation for every pixel in its input observations. PWVO employs uncertainty estimation to identify the noisy regions in the input observations, and adopts a selection mechanism to integrate pixel-wise predictions based on the estimated uncertainty maps to derive the final translation and rotation. In order to train PWVO in a comprehensive fashion, we further develop a data generation workflow for generating synthetic training data. The experimental results show that PWVO is able to deliver favorable results. In addition, our analyses validate the effectiveness of the designs adopted in PWVO, and demonstrate that the uncertainty maps estimated by PWVO is capable of capturing the noises in its input observations.

==> tables/big_table1.tex <==
\begin{table}[!htb]
    \begin{minipage}[t]{.5\linewidth}
        \centering
        \caption{ VONet egoloss depthloss PWVO }
        \resizebox{!}{10mm}{
            \begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
            \toprule
            & EPE & R err & T Err\\
            \hline
            \large{PWVO (M)} & 0.766 & 0.09 & 0.06\\
            \large{PWVO (P)} & 0.707 & 0.07 & 0.09\\ \\
            \large{PWVO (Ours)} & 0.626 & 0.08 & 0.04\\
            \toprule
            \end{tabular}
        }
        
    \end{minipage}%
    \begin{minipage}[t]{.4\linewidth}
        \centering
        \caption{Table 2}
        \resizebox{!}{12mm}{
            \begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
    
                % \cline{1-4}
                \toprule
                 & EPE & R Err & T Err\\
                \hline
                % pixel wise input total w/ rt unc + d unc + func
                \large{PWVO (M)} & 0.766 & 0.09 & 0.06\\
                % \hline
                % pixel wise input total w/ rt unc + d unc + func, patch select
                \large{PWVO (P)} & 0.707 & 0.07 & 0.09\\
                % \hline
                % pixel wise input total w/ rt unc + d unc + func, patch select soft
                \large{PWVO (PS)} & 0.626 & 0.08 & 0.04\\
                \toprule
            \end{tabular}
        }
    \end{minipage}
    
    \label{tab:big_table1}
\end{table}

==> tables/dataset_config.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|P{8mm}P{8mm}P{8mm}P{8mm}P{8mm}P{8mm}P{8mm}}
    \toprule
    Parameter & $\mu$ & $\sigma_{1}$ & $\sigma_{2}$ & k & $\rho$ & c & d \\
    \hline
    $R_{x}$ & 0.0 & 1.5 & 0.2 & 2.5 & 0.15 & -9.0 & 9.0\\
    $R_{y}$ & 0.0 & 2.0 & 0.2 & 2.0 & 0.15 & -9.0 & 9.0\\
    $R_{z}$ & 0.0 & 1.5 & 0.2 & 2.5 & 0.15 & -8.0 & 8.0\\
    $T_{x}$ & 0.0 & 0.4 & 0.03 & 2.5 & 0.15 & -0.7 & 0.7\\
    $T_{y}$ & 0.0 & 0.25 & 0.025 & 2.0 & 0.20 & -0.4 & 0.4\\
    $T_{z}$ & 0.0 & 1.80 & 0.02 & 2.5 & 0.15 & -5.0 & 5.0\\
    \toprule
\end{tabular}
\caption{Dataset Configuration }
\label{tab:config_table}
\end{table}

==> tables/experiment.tex <==
\begin{adjustbox}{max width=\textwidth}

\begin{tabular}{|l|P{20mm}|P{20mm}|P{15mm}|P{15mm}|P{15mm}|}
    % \cline{1-4}
    \hline
    % \multicolumn{1}{|c|}{} Dataset & Camera Motion & Depth Map & Flow  \\
    Setting & Motion Err. & R Motion Err. & T Motion Err. & Rotation Err. & \footnotesize{Translation} Err.\\
    \hline
    Stage I Dense(w/o ego)  &&&&&\\
    % Stage I Dense(w/o ego) & 1.365 & 0.584 & 1.391 & 0.103 & 0.064 \\
    % Stage I Conv(w/o ego) & 1.398 & 0.553 & 1.446 & 0.099 &0.059 \\
    Stage I Dense(w/ ego) & 0.909 &	0.568 &	0.859 & 0.11 & 0.0606 \\
    % Stage I Dense(w/ ego) & 1.001 & 0.543 & 1.046 & 0.112 & 0.068 \\
    % Stage I Conv(w/ ego) & 1.053 & 0.492 & 1.100 & 0.094 & 0.067 \\
    Stage I Dense (w/ ego, atten) & 0.894 & 0.558 & 0.855 & 0.117 & 0.076\\
    \hline
    Stage II(w/o ego)  &&&&&\\
    % Stage II(w/o ego) & 1.274 & 0.696 & 0.981 & 0.130 & 0.096 \\
    % Stage II(w/ ego) & 0.931 & \underline{$\textbf{0.387}$} & 0.994 & \underline{$\textbf{0.082}$} & \underline{$\textbf{0.046}$} \\
    Stage II(w/ ego) & 1.07	& 0.564	& 1.107 & 0.1063 & 0.0545 \\
    Best(w/ uncertainty) & 0.626 & 0.408 & 0.681 & 0.0806 & 0.0429 \\
    % Best(w/ uncertainty) & \underline{$\textbf{0.778}$} & 0.424 & \underline{$\textbf{0.898}$} & 0.088 & 0.058 \\
    \hline
\end{tabular}

\end{adjustbox}

==> tables/experiment2.tex <==
\begin{table*}[htbp]
\begin{adjustbox}{max width=\textwidth}
% \newcommand{\mytoprule}{\toprule[1.5pt]}

\begin{tabular}{l|P{8mm}|P{8mm}|P{12mm}|P{6mm}|P{11mm}|P{10mm}|P{10mm}|P{6mm}|P{9mm}|P{8mm}|P{8mm}}

    % \cline{1-4}
    \mytoprule
    % \hline
    % \multicolumn{1}{|c|}{} Dataset & Camera Motion & Depth Map & Flow  \\
     & Input & coord & Ego GT & PW & Unc RT & Unc D & Unc F & SM & M Err & R Err & T Err\\
    \hline
    \large{Stage I} & ego & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & 0.296 &	0.06 &	0.04\\
    % \hline
    \large{Stage I} & total & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark &0.909 &	0.11 &	0.06\\
    \large{Stage I} & total & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & 1.276 &	0.11 &	0.07\\
    \large{Stage I SA} & total & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & 0.894 & 0.558 & 0.855 \\
    \hline
    % pixel wise input ego
    \large{Stage II} & ego & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & M &0.263 &	0.05 &	0.02\\
    % \hline
    % pixel wise input total w/o ego supervision
    \large{Stage II} & total & \cmark & \xmark & \cmark & \xmark & \xmark & \xmark & M & 1.980 & 0.14	 & 0.07	\\
    % \hline
    % pixel wise input total
    \large{Stage II} & total & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & M &1.07 &	0.11 &	0.05\\
    % \hline
    % pixel wise input total w/ rt unc
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & M &0.829 &	0.09 &	0.06\\
    % \hline
    % pixel wise input total w/o ego supervision w/ rt unc
    % \large{Stage II} & total & \cmark & \xmark & \cmark & \cmark & \xmark & \xmark & M & 2.751  & 0.610	 & 2.778	\\
    % \hline
    % pixel wise input total w/ rt unc w/o coord
    \large{Stage II} & total & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & M &0.965 &	0.11 &	0.06\\
    % \hline
    % pixel wise input total w/ rt unc + d unc
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & M &0.729 &	0.09 &	0.08\\
    % \hline
    % pixel wise input total w/ rt unc + func
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \xmark & \cmark & M &0.768 &	0.09 &	0.09\\
    % \hline
    % pixel wise input total w/ rt unc + d unc + func
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & M &0.766 &	0.09 &	0.06\\
    % \hline
    % pixel wise input total w/ rt unc + d unc + func, patch select
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & P &0.707 &	0.07 &	0.09\\
    % \hline
    % pixel wise input total w/ rt unc + d unc + func, patch select soft
    \large{Stage II} & total & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & PS &0.626 & 0.08 & 0.04\\
    \large{Stage II SA} & total & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & PS &0.673 & 0.384 & 0.730\\
    \mytoprule
\end{tabular}

\end{adjustbox}
\caption{Train on 100k data samples.}
\label{tab:ablation_exp}
\end{table*}

==> tables/sintel.tex <==
\begin{table*}[htbp]
\begin{adjustbox}{max width=\textwidth}
\newcommand{\mytoprule}{\toprule[1.5pt]}

\begin{tabular}{l|P{9mm}|P{9mm}|P{8mm}|P{8mm}}

    % \cline{1-4}
    \mytoprule
    % \hline
     & Input & EPR & R_{Err} & T_{Err}\\
    \hline
    % eval on ego 
    VONet & Ego &  & 0.296 & 0.055 &	0.038\\
    VONet & Total & 0.513 &	0.086 &	0.057\\
    \hline
    PWVO w/o uncertainty  & Ego & 0.263 & 0.054 &	0.018\\
    PWVO w/o uncertainty  & Total & 0.757 & 0.097 &	0.052\\
    \hline
    PWVO (naive)  & Ego & 0.259 & 0.050 &	0.043\\
    PWVO (naive)  & Total & 0.526 & 0.072 &	0.057\\
    \hline
    PWVO & Ego & 0.187 & 0.037 &	0.022\\
    PWVO  & Total & 0.396 & 0.067 &	0.039\\
    \mytoprule
    % train with ego eval with total 
    VONet & Ego &  & 1.373 & 0.157 &	0.055\\
    PWVO w/o uncertainty  & Ego & 1.070 & 0.106 &	0.054\\
    PWVO (naive)  & Ego & 1.543 & 0.196 &	0.062\\
    PWVO & Ego & 1.490 & 0.174 &	0.043\\
    \mytoprule
\end{tabular}

\end{adjustbox}
\caption{Input representation.}
\label{tab:table_4}
\end{table*}

==> tables/table1.tex <==
\begin{table}[t]
\centering
\caption{Train on 100k data samples. SA: self-attention. cood: pixelwise coordinate. PW: pixelwise. Unc: uncertainty. SM: selection module. }
\begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
    \mytoprule
     & EPE & $R_{err}$ & $T_{err}$\\
    \hline
    \large{VONet~\citep{tartan}} & 0.909 & 0.110 & 0.061 \\
    \large{VONet + \textit{self-att.}~\citep{hamed2020attn}} & 0.894 & 0.117 & 0.076 \\
    \large{PWVO (\textit{base})} & 0.8829 & 0.09 & 0.06 \\
    \large{PWVO (\textit{final})} & \textbf{0.626} & \textbf{0.081}& \textbf{0.043} \\
    \mytoprule
\end{tabular}
\label{tab:table_1}
\end{table}

==> tables/table3.tex <==
\begin{table}[htbp]
\centering
\caption{Selection Module, M: Mean selection. P: Patch selection. PS: Patch Softmax selection}
\newcommand{\mytoprule}{\toprule[1.5pt]}
\begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
    
    % \cline{1-4}
    \mytoprule
     & EPE & $R_{err}$ & $T_{err}$\\
    \hline
    % pixel wise input total w/ rt unc + d unc + func
    \large{PWVO (M)} & 0.766 & 0.087 &	0.062\\
    % \hline
    % pixel wise input total w/ rt unc + d unc + func, patch select
    \large{PWVO (P)} & 0.707 &\textbf{0.073} & 0.091\\
    % \hline
    % pixel wise input total w/ rt unc + d unc + func, patch select soft
    \large{PWVO (PS)} & \textbf{0.626} & 0.081 & \textbf{0.043}\\
    \mytoprule
\end{tabular}
\label{tab:table_3}
\end{table}

==> tables/table4.tex <==
\begin{table*}[htbp]
\begin{adjustbox}{max width=\textwidth}
\newcommand{\mytoprule}{\toprule[1.5pt]}

\begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}

    % \cline{1-4}
    \mytoprule
    % \hline
    % \multicolumn{1}{|c|}{} Dataset & Camera Motion & Depth Map & Flow  \\
     & M Err & R Err & T Err\\
    \hline
    \large{VONet (Ego)} & 0.296 & 0.055 &	0.038\\
    % \hline
    \large{VONet (Total)} & 0.909 &	0.110 &	0.061\\
   
    \hline
    % pixel wise input ego
    \large{PWVO (Ego)} & 0.263 & 0.054 &	0.018\\
    % \hline
    % pixel wise input total w/o ego supervision
    \large{PWVO (Total)} & 1.070 & 0.106 &	0.055\\
    \mytoprule
\end{tabular}

\end{adjustbox}
\caption{Input representation.}
\label{tab:table_4}
\end{table*}

==> tables/table5.tex <==
\begin{table}[htbp]
\centering
\caption{Unc: Uncertainty.}
\begin{adjustbox}{max width=\textwidth}
\newcommand{\mytoprule}{\toprule[1.5pt]}
\begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
    % \cline{1-4}
    \mytoprule
    % \hline
    % \multicolumn{1}{|c|}{} Dataset & Camera Motion & Depth Map & Flow  \\
    \large{VONet} & M Err & R Err & T Err\\
    \hline
    % \hline
    % pixel wise input total
    \large{+ Pixel-Wise Prediction Stage} & 1.07 & 0.106 & 0.055\\
    \large{+ Unc RT} & 0.829 & 0.091 & 0.061\\
    \large{+ Unc D} & 0.729 & 0.089 & 0.082\\
    \large{+ Unc F} & 0.766 & 0.087 & 0.062\\
    % pixel wise input total w/ rt unc + d unc + func, patch select soft
    \large{+ Patch Selection} & 0.707 & \textbf{0.073} & 0.091\\
    \large{+ Patch Softmax Selection} & \textbf{0.626} & 0.081 & \textbf{0.043}\\
    \mytoprule
\end{tabular}
\end{adjustbox}
\label{tab:table_5}
\end{table}

==> tables/table6.tex <==
\begin{table}[t]
\centering
\caption{ }
\begin{tabular}{l|P{9mm}|P{8mm}|P{8mm}}
    \mytoprule
     & EPE & $R_{err}$ & $T_{err}$\\
    \hline
    \large{top 1} & 0.850 & 0.090 & 0.076 \\
    \large{all } & 0.690 & 0.077 & 0.041 \\
    \large{patch size = 16} & 0.567 & 0.075 & 0.051 \\
    \large{no depth loss} & 0.669 & 0.082 &  0.066\\
    \mytoprule
\end{tabular}
\label{tab:other_exp}
\end{table}
